PipeGCN: Efficient Full-Graph Training of Graph Convolutional Networks with Pipelined Feature Communication

Graph Convolutional Networks (GCNs) is the state-of-the-art method for learning graph-structured data, and training large-scale GCNs requires distributed training across multiple accelerators such that each accelerator is able to hold a partitioned subgraph. However, distributed GCN training incurs prohibitive overhead of communicating node features and feature gradients among partitions for every GCN layer during each training iteration, limiting the achievable training efficiency and model scalability. To this end, we propose PipeGCN, a simple yet effective scheme that hides the communication overhead by pipelining inter-partition communication with intra-partition computation. It is non-trivial to pipeline for efficient GCN training, as communicated node features/gradients will become stale and thus can harm the convergence, negating the pipeline benefit. Notably, little is known regarding the convergence rate of GCN training with both stale features and stale feature gradients. This work not only provides a theoretical convergence analysis but also finds the convergence rate of PipeGCN to be close to that of the vanilla distributed GCN training without any staleness. Furthermore, we develop a smoothing method to further improve PipeGCN's convergence. Extensive experiments show that PipeGCN can largely boost the training throughput (1.7x~28.5x) while achieving the same accuracy as its vanilla counterpart and existing full-graph training methods. The code is available at https://github.com/RICE-EIC/PipeGCN.

==> conclusion.tex <==
\section{Conclusion}
In this work, we propose a new method, PipeGCN, for efficient full-graph GCN training. 
PipeGCN pipelines communication with computation in distributed GCN training to hide the substantial communication overhead. Furthermore, 
we are the first to provide convergence analysis of GCN training with both stale features and feature gradients, and further propose a smoothing method to speedup the convergence of vanilla PipeGCN.
Extensive experiments validate the advantages of PipeGCN over both vanilla training (without staleness) and SOTA full-graph training. 


==> introduction.tex <==
\section{Introduction}

Graph convolutional networks (GCNs) \citep{kipf2016semi} have gained great popularity recently as they demonstrated the state-of-the-art (SOTA) performance in various graph-based learning tasks, including node classification \citep{kipf2016semi}, link prediction \citep{zhang2018link}, graph classification \citep{xu2018powerful}, and recommendation systems \citep{ying2018graph}.
The promising performance of GCNs is due to their diverse neighborhood connectivity, which provides a greater applicability to graph-based data than convolutional neural networks (CNNs) that adopt a fixed regular neighborhood structure.
In particular, a GCN aggregates all features from the neighbor node set for a given node, the feature of which is then updated via a multi-layer perceptron. 
Such a two-step process (i.e., \textit{aggregate} and \textit{update}) empowers GCNs to better learn graph structures.

However, training GCNs at scale has been a challenging problem, as a prohibitive amount of compute and memory resources are required to train a real-world large-scale graph, let alone exploring deeper and more advanced models.
To tackle this challenge, various sampling-based methods are proposed to reduce the resource requirement at a cost of incurring feature approximation errors.
A straightforward instance is to create mini-batches by sampling neighbors (e.g., GraphSAGE \citep{hamilton2017inductive} and VR-GCN \citep{chen2018stochastic}) or to extract subgraphs as training samples (e.g., Cluster-GCN \citep{chiang2019cluster} and GraphSAINT \citep{zeng2019graphsaint}). 

In addition to sampling-based methods, distributed GCN training has emerged as a promising alternative, as it enables large \textit{full graph} training of GCNs across multiple accelerators such as GPUs.
The essence of this approach is to separate a giant graph into several small partitions, each of which is able to fit into a single GPU, and then train these subgraphs locally on GPUs but with indispensable communication.
Following this direction, several recent works, including NeuGraph \citep{ma2019neugraph}, ROC \citep{jia2020improving}, and CAGNET \citep{tripathy2020reducing}, have been proposed and verified the great potential of distributed GCN training, e.g., demonstrating a better accuracy than the sampling-based methods~\citep{jia2020improving}.
Nonetheless, NeuGraph and ROC reply on CPUs to save the full graph with repeated swapping of subgraphs to GPUs for training, incurring a heavy CPU-GPU communication overhead; and
CAGNET distributes the large graph training based on matrix partitioning that introduces redundant broadcasts of node features and frequent synchronization.
Therefore, existing distributed training methods suffers either extra CPU swaps or redundant communication overhead, limiting their achievable training efficiency at scale.

In this work, we proposed a new method of distributed GCN training, PipeGCN, which targets achieving a full-graph accuracy with boosted training efficiency. Our main contributions are:
\begin{itemize}

    \item We first analyze two efficiency bottlenecks in distributed GCN training: \textit{significant communication overhead} and \textit{frequent synchronization}, and then propose a simple-yet-effective technique called PipeGCN to address the above two bottlenecks by pipelining inter-partition communication with intra-partition computation to hide the communication overhead.
	
	\item We address the challenge raised by PipeGCN, i.e., staleness in communicated features and feature gradients, by providing a theoretical convergence guarantee of PipeGCN which finds the convergence rate to be $\mathcal{O}(T^{-\frac{2}{3}})$, i.e., close to vanilla distributed GCN training without staleness.
	\textit{To the best of our knowledge, this is the first work providing theoretical proof for the convergence of GCN training with stale feature and feature gradients.}

	\item We further propose a low-overhead smoothing method to further improve PipeGCN's convergence by reducing the error incurred by the staleness.
	
	\item Extensive empirical and ablation studies consistently validate the advantages of PipeGCN over both vanilla distributed GCN training (boosting training throughput by up to 2.2$\times$ while achieving the same or a better accuracy) and SOTA full-graph training methods.  
\end{itemize}

